Textually Pretrained Speech Language Models

Speech language models (SpeechLMs) process and generate acoustic data only, without textual supervision. In this work, we propose TWIST, a method for training SpeechLMs using a warm-start from a pretrained textual language models. We show using both automatic and human evaluations that TWIST outperforms a cold-start SpeechLM across the board. We empirically analyze the effect of different model design choices such as the speech tokenizer, the pretrained textual model, and the dataset size. We find that model and dataset scale both play an important role in constructing better-performing SpeechLMs. Based on our observations, we present the largest (to the best of our knowledge) SpeechLM both in terms of number of parameters and training data. We additionally introduce two spoken versions of the StoryCloze textual benchmark to further improve model evaluation and advance future research in the field. We make speech samples, code and models publicly available: https://pages.cs.huji.ac.il/adiyoss-lab/twist/ .

==> RAI.tex <==
\section{Responsible AI}

SpeechLMs share the same potential benefits for society as text-based LMs as they give access, in the audio modality, to the same downstream applications (search, language generation, summarization, translation, chatbots, etc.), thereby increasing their reach to more use cases and more languages, including 'unwritten' (or sparsely written) languages \citet{on_generative}. As a result they also share the same potential risks regarding intentionally harmful applications (eg. fake news, spamming, election manipulation) or unintentionally harmful ones (e.g., unfair or biased results, toxic, regurgitated or untrustful generations). Assessing and mitigating these risks can be done with the same tools as for textLMs by translating the model's speech inputs and outputs into text using ASR and TTS. In Section \ref{sec:toxicity}, we provide an illustration of how this could be done by running the HolisticBias benchmark \cite{smith2022m} on our SpeechLM.   

In addition, Speech LMs carry risks that go beyond the risks traditionally associated with LMs. They are of three types, corresponding to the three components of current speechLMs: Risks associated with the speech tokenizer, with the token-to-speech generator (synthetizer), and with the token-fed language model.  

The risks associated to the \textit{speech tokenizer} are similar to the ones associated to traditional ASR: the quality of the tokens may be affected by the distribution of the data in the training set, and therefore show \textbf{lack of robustness} and \textbf{bias} with respect to recording conditions, voice types, speaking styles or accents that are less represented in the training set \cite{riviere2021asr4real,aksenova2022accented,dheram2022toward}. Mitigation measures for this risk would include increasing the size of the dataset, compensating for bias in representation of different demographics, and making the tokenizer robust to a representative variety of recording conditions. In Section \ref{sec:ASR4real}, we apply ASR4real \cite{riviere2021asr4real}, a benchmark for measuring bias in ASR systems which we adapt to be used with our speechLM. An additional risk associated to the speech tokenizer is that it may leak partial information about the identity of the speaker, or at least some of its characteristics (like gender, accent and expressive contents) \cite{sicherman2023analysing,de2022probing}. This leakage in itself may be harmful, but needs to be taken in consideration regarding what the LM learns from these tokens and how the synthetizer renders them.

The risks associated to the \textit{speech synthetizer} depend on how the voices of the synthetizer were obtained. 

If the synthetizer uses a fixed set of pretrained voices, and assuming the content and license allows for such usage, the main risk mirrors that of the tokenizer: the synthetizer's performance depends on its training set. If certain voice types or vocalizations are tokenized with tokens that are not present in the synthetizer's training set, it will not be able to render them. Mitigation for this risk consists in matching the distribution of tokens in the training set of the LM and of the voice dataset, and more generally to have the most diverse and expressive set of voices possible to train the synthetizer (see the Expresso paper)\footnote{The choice of the dialects and voices types used to train the synthetizer is itself of ethical import depending on the application. If several dialects are included in the training set, it is important to study how faithfully and respectfully they are rendered in the synthetizer.}. In Section \ref{sec:ASR4real}, we evaluate both risks at the same time, since ASR4real is applied to the pipeline tokenizer+synthetizer, and we compute the WER on the resynthetized speech. This enables us to assess the global risk of bias regarding recording conditions, voice type and dialect (although does not provide a diagnostic regarding which part of the pipeline is at fault). 

If the synthetizer is conditioned on a voice embedding, it can potentially do voice cloning, ie, generate speech in the voice of any chosen individual. This carries the additional risk of impersonating, fake news, or non-consensual spoken content generation. We do not use this technique in our speechLM as, in our opinion, the risks outweigh the benefits.

The risks associated to the \textit{language model} depend on the degree of voice leakage at the tokenizer level. For instance, if the tokenizer uses different tokens for males and female speakers, then the LM becomes aware of that factor and may learn some of the gender biases that are present in the training set. As the result, it may produce biased content prompted by different input voices, in a way that would not be detected by traditional text-based methods. Completely new tools need to be built to study how sociolinguistic factors are passed on to the language model, and how they may bias generated content, including accent mockery, voice-conditioned social bias, etc.

\subsection{Toxicity}\label{sec:toxicity}

For toxicity analysis we randomly selected 250k Holistic Bias prompts \cite{smith2022m} which consists of over 472k English sentences (e.g., “I am a disabled parent.”) used in the context of a two-person conversation and representing 13 demographic axes. This dataset does not contain toxicity inputs according to the ETOX toxicity classifier \cite{costajussa2023}. However, previous work \cite{costajussà2023} has shown that \textsc{holisticbias} provides a good setting for analyzing added toxicity. Then, we generated speech from these prompts using the open-source TTS\footnote{https://github.com/facebookresearch/fairseq/blob/main/examples/speech_synthesis/docs/ljspeech_example.md#results}. Then, we prompted our model using this prompts {\color{red} Tal should provide details}. The output of these generations was transcribed using Whisper\footnote{https://huggingface.co/openai/whisper-large}. Finally, we ran ETOX on these transcriptions and we computed {\color{red} XX} toxicity detections. This provides a simple quantification of our model's toxicity for this particular experimental setting. In the future, we can analyse how toxicity is related to the different demographic axes of HolisticBias.

\subsection{Tokenizer \& Synthetizer Bias}\label{sec:ASR4real}

Here, we use the ASR4Real dataset to test for bias in how speech is being encoded into tokens or tokens being decoded into speech. Bias can arise in these two processes for reasons that mirror one another. During encoding, meaningful phonetic distinctions may be coded into the same token representation, yielding confusions for downstream processing. This may happen in particular for speech which distribution was not sufficiently represented during the training of the Hubert units. It is also possible that tokens encode non meaningful phonetic distinctions and leak characteristics of the speakers by giving groups of speakers different units. During decoding, these variations may not be correctly rendered into speech if they were not present in the training set of the synthetizer. Here, we evaluation these two problems at once, by piping encoding and decoding in a speech resynthesis task. In this task, the model is presented wit speech, encodes it into tokens and reconstruct speech with one of the synthetizer's voice. The result is then fed to an ASR system (whisper), and a WER is computed. 

We test the two tokenizers that gave the best results: Hubert200 with 50Hz units and Hubert500 with 25Hz units. We also provide the ASR results with the raw audio, as this gives a baseline estimation of the bias inherent to our ASR measuring instrument. In Table \ref{tab:ASR4real}, we show the WER in 5 datasets spanning 3 styles (read, formal, and conversational speech) and a variety of accents and socio-economic status as available in the AllStar, NISP, VoxPopuli, Buckeye and Coraal datasets used in ASR4real.


\begin{table}[]
\caption{}\label{tab:ASR4real}
\begin{tabular}{l cccc cccc cccc}
\hline
          & \multicolumn{4}{c}{raw audio} & \multicolumn{4}{c}{Hub200 50Hz} & \multicolumn{4}{c}{Hub500 25Hz} \\
Dataset   & med   & p90   & top   & bot   & med   & p90   & top   & bot   & med   & p90   & top   & bot   \\
\hline
\multicolumn{13}{c}{Read Speech}                                                                          \\
ALLStar   &       &       &       &       &       &       &       &       &       &       &       &       \\
NISP      &       &       &       &       &       &       &       &       &       &       &       &       \\
\multicolumn{13}{c}{Formal Speech}                                                                        \\
VoxPopuli &       &       &       &       &       &       &       &       &       &       &       &       \\
\multicolumn{13}{c}{Conversational Speech}                                                                \\
Buckeye   &       &       &       &       &       &       &       &       &       &       &       &       \\
Coraal    &       &       &       &       &       &       &       &       &       &       &       &      \\
\hline
\end{tabular}
\end{table}

==> old-06_results.tex <==
\section{Results}
\label{sec:res}

We start by evaluating the effect of the speech tokenizers on the overall system performance. For each token type, we train two \slms based on the OPT350M model. The first one is randomly initialized, while the second one follows the \method approach, denoted as \textsc{Rand.} and \method respectively. Results are reported in \cref{tab:tok}.

\begin{figure*}[t!]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]
         {figs/size_fig_special.pdf}
         \caption{\label{fig:size}}         
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/train_fig_special.pdf}
         \caption{\label{fig:train_curve}}         
     \end{subfigure}
     \caption{In (a) \ac{PPL} as  a function of training data set for 25Hz tokens. Results are reported for different model scales, with and without text pretraining. (b) valid \ac{PPL} as a function of training steps. \roy{missing take home message}\label{fig:ppl_scaling}   }
\end{figure*}

We observe a consistent improvement across all metrics following the \method approach. Interestingly, when speech units with larger downsampling factor (.i.e., smaller frequency) leads to significantly better sWUGGY and sBLIMP. This findings are consistent with \cite{borsos2022audiolm}.

For the rest of the paper we report results using the speech tokenizer with 500 tokens at 25Hz which gets the best sWUGGY and sBLIMP results. This is also being reflected by the speech resynthesis results, see \cref{tab:tok_re} in the Appendix. 

As prior work mainly considered relatively small \ac{LM}s (e.g., $\sim$100M parameters in~\cite{on_generative, kharitonov2021text}) and relatively small training data (e.g., \cite{borsos2022audiolm} use Librilight only), in the following we evaluate the effect of model and dataset scaling on the overall performance. 

As mentioned we train three different \slms using the OPT family. For each model size, we increase the magnitudes of training data, considering 1$\%$, 10$\%$, and 100$\%$ of the training data with and without initializing from a text-based \ac{LM}. \cref{fig:size} and \cref{fig:size_fig_50hz} depicts the \ac{PPL} of the various evaluated configurations. Results suggest that \slms initialized from a text-based \ac{LM} performs consistently better, while as expected with increasing the magnitude of the dataset all models get better. The full set of results, i.e., sWUGGY, sBLIMP, text-PPL and text-aBLEU for the corresponding models can be found on \cref{tab:scale} in \cref{app:...} \tal{supplementary metrial}. 

Next, we analyze how pretraining affects model convergence. \cref{fig:train_curve} presents the validation loss training curves for a \method-350M models. It can be seen that when starting from a pretrained text \ac{LM}, the model reaches the same \ac{PPL} in about quarter of the training updates.

Lastly, we report results for different \ac{LM} model architecture, i.e., Bloom~\citep{scao2022bloom} and Pythia~\citep{biderman2023pythia}, and different modality pretraining using ImageGPT~\citep{chen2020generative}. Results are reported in \cref{tab:arch,tab:modality} in \cref{sec:lm_arch,sec:pre_mod}. We observe similar trends in Bloom and Pythia, in which textually pretraining yields better results. When considering other modalities for pretraining, interestingly, ImageGPT pre-trained models perform significantly worse than models pretrained on text. For a reference, models trained from scratch achieve comparable performance to previously reported models.

\begin{table}[t!]
\caption{Results are reported for the \method-7B model, 200 units sampled at 50Hz, and 500 units sampled at 25Hz. We report sWUGGY, sBLIMP,  PPL over the transcribed text (\textsc{text-PPL}), and diversity metric over the transcribed text using the auto-BLEU metric (\textsc{text-aBLEU}). \label{tab:llms}}  
\centering
\begin{tabular}{lccccc}
    \toprule
    \textsc{Tokens freq.} & \textsc{sWUGGY}$\uparrow$ & \textsc{sBLIMP}$\uparrow$ & \textsc{text-PPL}$\downarrow$ & \textsc{text-aBLEU}$\downarrow$ \\
    \hline
    van Niekerk et al.  & 72.3  & 54.0           & - & - \\
    GSLM                & 68.7  & 57.1          & - & - \\
    AudioLM             & 83.7  & \textbf{64.7} & - & - \\
    \hline
    \method-7B & \textbf{84.4} & 62.1 & 65.21 & 0.22 \\
    \bottomrule
\end{tabular}
\end{table}


\subsection{Speech Large Language Models}

Equipped with previous findings in this sub section we report a 7B parameter \slm initialized from the LLaMA-7B model, denoted as \method-7B. In \cref{tab:llms} we report the full set of results for the \method-7B models. As expected, when initializing the models from LLaMA, we observe an additional improvement across all metrics. When comparing to \method-1.3B, we do observe a significant improvement comparing to previous settings ($\sim$8$\%$ relative improvement). When using speech units at 25Hz, we observe another significant boost in performance, reaching sWUGGY of 84.36 ($\sim$10$\%$ improvement), and sBLIMP of 62.11 ($\sim$2$\%$ improvement). This additionally suggests that the granularity of the speech tokens has great impact of these metrics. 


\subsection{Spoken StoryCloze.}
To better asses the contextual understanding the \slms we conduct an additional set of experiments using the newly created Spoken StoryCloze (see \cref{sec:eval} for more details regarding dataset creation). 

\begin{wraptable}{r}{0.5\textwidth}
\caption{Results for spoken \tsc benchmark.\label{tab:story}} 
\centering
\resizebox{0.42\textwidth}{!}{%
\begin{tabular}{lcc}    
    \toprule
    \textsc{Model} & \textsc{Freq.} &\textsc{Acc. ($\%$)}$\uparrow$ \\
    \hline
    LLaMA-7B-text & - & 98.3 \\
    \hline
    GSLM-1.3B & \multirow{3}{*}{50Hz} & 53.9  \\
    \method-1.3B & & 54.9 \\
    \method-7B &  & \textbf{56.5} \\
    \hline
    GSLM-1.3B & \multirow{3}{*}{25Hz} & 60.1  \\
    \method-1.3B & & 61.3 \\
    \method-7B &  & \underline{\textbf{64.4}} \\
    \bottomrule
\end{tabular}}
\end{wraptable}

In initial experimentation we found the \ssc benchmark is extremely challenging, for \slms. Most of the evaluated models performs slightly above change level. Notice, this task is also challenging to text-based models. Following our evaluation method, the LLaMA-7B model reaches~80$\%$. Considering the fact that both models operate on completely different units granularity (subwords vs.~pseudo phoneme-states), such results are expected. When considering \tsc, which measures sentence coherence in terms of overall sentence topic, as expected, text based models reach almost perfect scores. \method-7B reaches the best scores across all models. We do see an improvement following the \method approach, with models pretrained on text data. The results are summarized in \cref{tab:story}.


\subsection{Human Evaluation.}
We conclude with a human evaluation. We randomly sample a collection of 50 examples from the test sets of 3 different datasets: LibriLight, LibriSpeech-Clean and LibriSpeech-other to reach overall 150 samples per evaluated method. We evaluate the following models: \method-1.3B with and without text pre-training using 200 tokens at 50Hz, \method-7B with pre-training using both 200 units at 50Hz and 500 units at 25Hz, and resynthesized audio samples using both 200 at 50Hz and 500 at 25Hz. The resynthesis scores serve as a top-line estimate together with the reference audio recordings. Results are visually depicted in \cref{fig:mmos}.

\begin{figure*}[t!]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/mos_ls_clean.pdf}
         \caption{Libri-Speech Clean.\label{fig:mos_ls}}         
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/mos_ls_other.pdf}
         \caption{Libri-Speech Other.\label{fig:mos_ls_o}}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/mos_ll.pdf}
         \caption{Libri-Light.\label{fig:mos_ll}}
     \end{subfigure}
     \caption{Meaningfulness results for different models. Results are reported for a subset from Libri-Speech Clean, Libri-Speech Clean, and Libri-Light.\label{fig:mmos}}
\end{figure*}

Results suggest that using \method-7B with 500 sampled at 25Hz and \method-7B with 200 units sampled at 50Hz performs comparably, while both are superior to the \method-1.3B model. The models which are not initialized from text models perform consistently worse. Interestingly, we did not observe significant differences between the evaluated datasets. Examples of generated sentences can be seen on \cref{fig:text_gen_prompt}.

\begin{figure*}[t!]
     \centering    
      \includegraphics[width=\textwidth]{figs/text-fig.pdf}
      \caption{Example generations for two different prompts using \method-1.3B, both pretrained on text and randomly initialized, together with \method-7B. We additionally provide the original text as reference \michael{let's find a better cherry picked example. maybe from an easy to read prompt?}.\label{fig:text_gen_prompt}}
\end{figure*}


==> old_04_method.tex <==
\section{Method}
\label{sec:method}


In this work, we study the effect of training SpeechLMs using spoken data initialized from a pretrained text LM. We denote this method \teps. Specifically, we leverage pre-trained text language models e.g., Bloom~\citep{scao2022bloom}, LLaMA~\citep{touvron2023llama}, and use them as initialization point for training using speech tokens.

\begin{wrapfigure}{r}{0.5\textwidth}
    \vspace{-15pt}
    \centering 
    \includegraphics[width=0.48\textwidth]{figs/fig_1.pdf}
    \caption{A visual description of the proposed method. We initialize a SpeechLM model from a pretrained text LM. \label{fig:method}}
    \vspace{-15pt}
\end{wrapfigure}

In this work, we propose to construct a SpeechLM from a pre-trained text LM and fine-tune the model using spoken data. For that, we change the vocabulary, $\mathcal{W}$, to be $\mathcal{Z}$, (the set of speech tokens defined in Section~\ref{sec:back}) and set the tokenizer to be a speech based tokenizer. We replace the text lookup table with a new randomly initialized embedding table for the speech tokens. The rest of the body of the network remains unchanged during initialization time. A visual description can be found in Figure~\ref{fig:method}. 

One might wonder, whether such an approach would make sense as speech tokens operate on 20-40ms windows while text tokenizers span significantly bigger concepts (e.g., sub-words). However, although being simple, interestingly we observe consistent improvement in performance across all evaluated setups. The study of  advanced methods for converting speech tokens to word tokens is deferred to future work. %




==> old_05_exp.tex <==
\section{Experimental Setup}
\label{sec:exp}
We follow the same setup as described in \cref{sec:back}. Similarly to~\cite{on_generative}, we consider HuBERT~\citep{hubert} followed by a k-means quantizer as the speech tokenizer model. For the Unit-to-speech model, we use a unit based HiFi-GAN neural vocoder with duration predictor as in~\cite{polyak2021speech, lee2021direct}. Then we optimize, compare and analyze the performance of various \slms considering different setups. 

\subsection{Datasets}
\label{sec:data}
All \slms are optimized using a collection of publicly available academic speech datasets. Specifically, we use Librispeech~\citep{librispeech}, LibriLight~\citep{kahn2020libri}, Spotify podcasts~\citep{clifton2020spotify}, People dataset~\citep{galvez2021people}, and VoxPopuli~\citep{wang2021voxpopuli}. We filter non-English data using the provided meta-data. This results in $\sim$150k hours, which translate to 13.52B tokens when using a token frequency of 50Hz and 9B tokens using a token frequency of 25Hz \tal{I would add a footnote that explains the 25Hz is not hald of the 50Hz tokend due to deduplication. Otherwise this just seems like an error.}. See \cref{tab:db_stats} for detailed descriptions of the datasets. To the best of our knowledge, this is the first work that uses this scale of data to train \slms.

\begin{table}[t!]
    \centering  
    \caption{Speech datasets statistics. We report both the number of hours in the training data of each dataset together with the number of speech tokens used to train the speech language model.\label{tab:db_stats}}%
    \begin{tabular}{lcccccc}
    \toprule
    & \small \textsc{LibriSpeech} & \small \textsc{LibriLight} & \small \textsc{Spotify} & \small \textsc{People} & \small \textsc{VoxPopuli} & \small \textsc{Overall}\\
    \midrule
    Hours  & \phantom{0}960 & \phantom{00}53k & \phantom{00}59k & \phantom{00}17k & \phantom{00}20k & \phantom{00}150k \\
    Tokens-50Hz & 86M & 4.79B & 5.34B & 1.54B & 1.76B & 13.52B \\
    Tokens-25Hz & 58M & 3.19B & 3.56B & 1.02B & 1.17B & 9.00B \\
    \bottomrule
    \end{tabular}      
\end{table}

In cases where no pre-defined validation and test sets are available, we randomly sample 2\% of the data serving as validation set and additional 2\% for the test set. Unless stated otherwise, in all setups reported results are the average across all different datasets.


\subsection{Model $\&$ Hyperparameters} 

Our main family of transformer models is OPT~\citep{zhang2022opt}. We examine three model sizes: OPT-125M, OPT-350M and OPT-1.3B, where each model has 12/24/24 transformer blocks and 768/1024/2048 hidden dimension, respectively.\footnote{The actual number of parameters of the speech models is actually about 10/15/25\%  lower from the text ones since we are replacing the text embedding layer with smaller speech embedding layer.}  We also experiment with Bloom \citep{scao2022bloom} and Pythia \citep{biderman2023pythia} (with equivalent sizes to OPT-350M) to consider other transformer architectures, and for the scaling experiments we use the recent LLaMA-7B model \citep{touvron2023llama}. For each model size, we compare two variants: \method, i.e., a warm initialization from a textual \ac{LM}, and a cold (randomly initialized) model following the original \ac{GSLM} approach.

We train our models (non LLaMA) with a batch size of 64, where each sample is bounded for 25 seconds and 704 tokens. The models are trained for 400k steps ($\sim$1.2 epochs), using an inverse-sqrt scheduler, 100 warmup steps and wADAM as the optimization algorithm. We also tune the learning rate per scenario, i.e: using/not-using pretrained LM, we end up with a maximal learning rate of 4e-4/8e-5 and final learning rate of 8e-5/2.5e-5, respectively.
We use 8 GPUs for training except for the 1.3B models, which use 32 GPUs.
As for LLaMA models, we use same configurations except the following: cosine learning rate schedule, 500 warmup steps, a maximum learning rate of 1e-4 and a final rate of 1e-5, batch size of 1024 over 32 GPUs for 75k steps ($\sim$4 epochs). In all cases we choose the best checkpoint by the speech perplexity of the model over the validation set.

For the speech tokenizers, we quantize HuBERT representations, operates at 50Hz, with 100, 200, and 500 clusters using the k-means algorithm. HuBERT is trained on Librispeech 960h while k-means are trained over the `clean-100h' part only from the Librispeech corpus. All models and quantizers are obtained from the textless-lib~\citep{kharitonov2022textless}. Inspired by~\cite{chung2021w2v} and~\cite{borsos2022audiolm}, we also trained a new HuBERT tokenizer with a lower sampling rate. We trained the HuBERT model on a varied mixture of datasets: Multilingual LibriSpeech~\citep{pratap2020mls}, Vox Populi~\citep{wang2021voxpopuli}, Common Voice~\citep{ardila2019common}, Spotify~\cite{clifton2020spotify}, Fisher~\citep{cieri2004fisher}. The model was trained for 3 iterations with the default 50Hz features rate. For the 4-th iteration, we add an additional convolutional layer at the CNN Encoder with the strides 2/3/4, resulting in features of 25Hz/16.6Hz/12.5Hz, respectively. Our early ablations show that 25Hz features with 500 tokens give the best results in terms of language modeling, we thus trained our models on these new tokens and compare them with the rest of the tokens. \tal{Let's refer to the supplamentry meterial Table 5.}

\subsection{Evaluation}
\label{sec:eval}
Evaluating such a complex pipeline comprised of several different components is a challenging task. \citet{on_generative} were the first to propose a set of evaluation metrics. We follow such an approach and augment it with the StoryCloze evaluation benchmark. Overall, we consider five different axis for evaluation: (i) Resynthesis; (ii) Zero-shot modeling; (iii) Generation and diversity; (iv) Human evaluation; and (v) Spoken StoryCloze. 

\noindent {\bf Resynthesis metrics} does not involve\slms, and measure our ability to fully recover the speech content after tokanization. As we additionally evaluate several speech tokenizers, we provide resynthesis metrics in the form of \ac{WER} together with \ac{PPL} and auto-BLEU over the transcribed text~\citep{on_generative}. We use Whisper~\citep{radford2022robust} ``small'' as our \ac{ASR} model. To measure \ac{PPL} we use the LLaMA-7B model (in its text form). For the auto-BLEU metric we follow \cite{on_generative} and use 3- and 4-grams. We evaluate 3,072 examples, with 8 seconds (or more) length, from the Librispeech-Clean, Librispeech-Other and LibriLight test sets (1,024 example from each dataset). These metrics serve as an upper bound on the performance of \slms as they reflect the information loss due to tokanization and speech synthesis.

\noindent {\bf Zero-shot metrics.} We use the sWUGGY and sBLIMP~\citep{nguyen2020zero} metrics to evaluate lexical and syntactic modeling of the \slms. In sWUGGY, the network is presented with a pair of utterances, an existing word and a matching non-word, and are evaluated on their capacity to attribute a higher probability to the existing
word. As for sBLIMP, similarly to sWUGGY, the network is presented with a matched pair of speech segments, grammatical and ungrammatical sentences. The task is to decide which of the two is grammatical based on the probability of the sentence. We additionally report speech tokens \ac{PPL} (average across all datasets). Notice, although \ac{PPL} is not comparable across different tokenizers, it can be helpful to compare \method vs. randomly initialized models.

\noindent {\bf Generation and diversity metrics.}
 We report auto-BLEU~\citep{on_generative} and text-\ac{PPL} measured over the transcribed text (same as mentioned above). In preliminary experiments, we notice errors from the \ac{ASR} model such as word corrections for unintelligible speech, can affect the text-\ac{PPL} metric. To mitigate that, we propose to first calibrate the temperature parameter using the \ac{ASR} probability for a given speech utterance with respect to the original recordings. This can be interpreted as the ASR confidence in the transcribed text. 
  
  Next, we calibrate the temperature according to the auto-BLEU metric with respect to the original text transcriptions (using the validation set). This process allows us to find near-optimal temperatures for generating high-quality speech while maintaining similarity to the reference text in terms of diversity. Finally, both text-\ac{PPL} and auto-BLEU scores for the generated samples over the transcribed speech are reported to present the trade-offs between generation quality and diversity. 

\noindent {\bf Human evaluation.} We follow the same setup as the Meaningfullness MOS (MMOS) in~\cite{on_generative}. In which, raters are presented with several speech continuations (each $\sim$10 seconds long) following the same speech prompt, and are instructed to evaluate how natural (considering grammar, meaning, and diversity) a given sample is, on a scale between 1-5 with an increment of 0.5.  We enforce 10 raters per sample and use the CrowdMOS~\citep{ribeiro2011crowdmos} package with the recommended recipes for detecting and discarding inaccurate scores.

\begin{table}[t!]
  \caption{Speech Continuation results\tal{shouldnt this table be called "Tokenizer effect"? or something of that sort?}. Results are reported for different number of units and downsampling factors (Frequency), with and without textual pretraining (\textsc{Pre.}). We report PPL over speech units, sWUGGY, sBLIMP,  PPL over the transcribed text (\textsc{text-PPL}), and diversity metric over the transcribed text using the auto-BLEU metric (\textsc{text-aBLEU}). Bold indicates the best model for each tokenizer, and we underline the best performing model overall.\label{tab:tok}}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{cccccccc}
    \toprule
    \textsc{Model} &
    \textsc{\# units} & \textsc{Freq.} &  \textsc{PPL}$\downarrow$ & \textsc{sWUGGY}$\uparrow$ & \textsc{sBLIMP}$\uparrow$ & \textsc{text-PPL}$\downarrow$ & \textsc{text-aBLEU}$\downarrow$\\
\hline
GSLM & \multirow{2}{*}{100} & \multirow{2}{*}{50Hz}	&	5.26	&	68.33	&	55.42	&	35.42	&	0.43	\\ 
TWIST & & &	\textbf{5.03}	&	\textbf{70.30}	&	\textbf{57.51}	&	37.51	&	0.38	\\
\hline
GSLM & \multirow{2}{*}{200}	& \multirow{2}{*}{50Hz} &	5.61	&	68.68	&	55.55	&	39.21	&	0.37	\\
TWIST &  & &	\textbf{5.29}	&	\textbf{71.83}	&	\textbf{57.89}	&	77.72	&	0.28	\\
\hline
GSLM & \multirow{2}{*}{500}	& \multirow{2}{*}{50Hz} &	6.36	&	67.24	&	53.20	&	83.95	&	0.37	\\
TWIST &  & &	\textbf{5.85}	&	\textbf{71.05}	&	\textbf{55.05}	&	66.25	&	0.31	\\
\hline
GSLM & \multirow{2}{*}{500}	& \multirow{2}{*}{25Hz} &	6.65	&	80.38	&	57.99	&	117.12	&	0.27	\\
TWIST &  &	&	\textbf{6.25}	&	\underline{\textbf{82.41}}	&	\underline{\textbf{59.31}}	&	92.69	&	0.25	\\
    \bottomrule
  \end{tabular}}
\end{table}

\noindent {\bf Spoken StoryCloze.}
Finally, to better evaluate the capabilities of the proposed \slms in capturing fine-grained textual nuances and continuation coherence, we provide two spoken versions of the StoryCloze textual benchmark~\citep{mostafazadeh2016corpus}, denoted by Spoken StoryCloze (\ssc) and Topic StoryClose (\tsc). The textual StoryCloze benchmark contains~4k five-sentence commonsense stories (split to validation and test sets). For each story, there is an additional negative sample, composed of the first four sentences followed by a negative continuation (ending sentence). The goal is to distinguish the original fifth sentence from the negative one. To generate the spoken benchmark, we synthesize the stories from the test set using a single speaker TTS system as provided by~\cite{wang2021fairseq} comprised of a FastSpeech2.0~\citep{ren2020fastspeech} model and HiFi-GAN vocoder~\citep{kong2020hifi}.\footnote{We introduce a 100ms of silence between segments to generate naturally spoken sentence.} 

For \ssc, we follow the original StoryCloze negative samples. With this benchmark, we evaluate the models capabilities to capture fine-grained causal and temporal commonsense relations. For \tsc, we randomly sample the negative ending sentence from the dataset. The premise behind \tsc is to evaluate continuation coherence given a spoken prompt. This version is far easier, but our experiments show that it is still quite challenging for modern \slms. Similar to sWUGGY, we feed  both speech segments to the \slm, measure the probability of each spoken sentence, and report the percentage of examples where the probability of the positive sample is higher than the negative one. \tal{we can say here we will release all the audio files.}
